Distributed Recursion Revisited

The distributed recursion (DR) algorithm is an effective method for solving the pooling problem that arises in many applications. It is based on the well-known P-formulation of the pooling problem, which involves the flow and quality variables; and it can be seen as a variant of the successive linear programming (SLP) algorithm, where the linear programming (LP) approximation problem can be transformed from the LP approximation problem derived by using the first-order Taylor series expansion technique. In this paper, we first propose a new nonlinear programming (NLP) formulation for the pooling problem involving only the flow variables, and show that the DR algorithm can be seen as a direct application of the SLP algorithm to the newly proposed formulation. With this new useful theoretical insight, we then develop a new variant of DR algorithm, called penalty DR (PDR) algorithm, based on the proposed formulation. The proposed PDR algorithm is a penalty algorithm where violations of the (linearized) nonlinear constraints are penalized in the objective function of the LP approximation problem with the penalty terms increasing when the constraint violations tend to be large. Compared with the LP approximation problem in the classic DR algorithm, the LP approximation problem in the proposed PDR algorithm can return a solution with a better objective value, which makes it more suitable for finding high-quality solutions for the pooling problem. Numerical experiments on benchmark and randomly constructed instances show that the proposed PDR algorithm is more effective than the classic SLP and DR algorithms in terms of finding a better solution for the pooling problem.

==> section_equivalence-arXiv.tex <==
\section{Equivalence of the \DR and \SLP approaches}
\todo[inline]{YW: The title need to be re-considered.}





%\subsection{Distributive Recursion (\DR) approach for solving $P$-formulation} \label{subsect:DR}
%\todo[inline]{YW: We first consider how to transform the first-order approximation of constraint \eqref{cons:material-balance-ell} and \eqref{cons:material-balance-j-lb}--\eqref{cons:material-balance-j-ub} by utilizing $(\alpha^\ast, y^\ast)$.}
%Let $(\alpha^\ast, y^\ast)$ be a solution of problem \eqref{prob:pooling-P} such that equations \eqref{cons:material-balance-ell} hold:
%\begin{equation}\label{cons:material-balance-ell-star}
%	\sum_{i \in I} \lambda_{ik} y_{i\ell}^\ast
%	= \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j}^\ast, \ \forall \ \ell \in L, \ k \in K. 
%\end{equation}
%%\todo[inline]{YW: Note that solution $(\alpha^\ast, y^\ast)$ may not satisfy other constraints in problem \eqref{prob:pooling-P}.}
%We consider the following approximated equations of \eqref{cons:material-balance-ell} by performing the first-order Taylor's expansion at point $(\alpha^\ast, y^\ast)$:
%\begin{equation}\label{cons:material-balance-ell-approx} \small
%	\sum_{i \in I} \lambda_{ik} y_{i\ell}
%	= \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j}^\ast 
%	+ \alpha_{\ell k}^\ast \left(\sum_{j \in J} y_{\ell j} - \sum_{j \in J} y_{\ell j}^\ast \right)
%	+ \left(\alpha_{\ell k} - \alpha_{\ell k}^\ast \right) \sum_{j \in J} y_{\ell j}^\ast, \ \forall \ \ell \in L, \ k \in K, 
%\end{equation}
%Similarly, we approximate inequalities \eqref{cons:material-balance-j-lb}--\eqref{cons:material-balance-j-ub}, obtaining 
%\begin{subequations}
%	\begin{align}
%		& \sum_{i \in I} \lambda_{ik} y_{ij}
%		+ \sum_{\ell \in L} 
%		\left( 
%			\alpha_{\ell k}^\ast y_{\ell j}^\ast 
%			+ \alpha_{\ell k}^\ast ( y_{\ell j} - y_{\ell j}^\ast)
%			+ (\alpha_{\ell k} - \alpha_{\ell k}^\ast) y_{\ell j}^\ast
%		\right)
%		\ge \lambda_{jk}^{\min} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K,
%		\label{cons:material-balance-j-lb-approx}\\
%		& \sum_{i \in I} \lambda_{ik} y_{ij}
%		+ \sum_{\ell \in L} 
%		\left( 
%			\alpha_{\ell k}^\ast y_{\ell j}^\ast 
%			+ \alpha_{\ell k}^\ast ( y_{\ell j} - y_{\ell j}^\ast)
%			+ (\alpha_{\ell k} - \alpha_{\ell k}^\ast) y_{\ell j}^\ast
%		\right) 
%		\le \lambda_{jk}^{\max} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K.
%		\label{cons:material-balance-j-ub-approx}
%	\end{align}
%\end{subequations}
%For simplicity of notations, we denote the first order Taylor's expansion of the bilinear term $\alpha_{\ell k} y_{\ell j}$ at point $\alpha_{\ell k}^\ast y_{\ell j}^\ast$ by $\widehat{\alpha_{\ell k} y_{\ell j}}$ for all $\ell \in L$, $k \in K$, and $j \in J$, i.e., 
%\begin{equation}
%	\widehat{\alpha_{\ell k} y_{\ell j}} := 
%	\alpha_{\ell k}^\ast y_{\ell j}^\ast 
%	+ \alpha_{\ell k}^\ast ( y_{\ell j} - y_{\ell j}^\ast)
%	+ (\alpha_{\ell k} - \alpha_{\ell k}^\ast) y_{\ell j}^\ast
%	= \alpha_{\ell k}^\ast y_{\ell j} + (\alpha_{\ell k} - \alpha_{\ell k}^\ast) y_{\ell j}^\ast.
%\end{equation}
%Given $\ell \in L$ and $k \in K$, we consider the following two cases.
%If the total amount of outflow at pool node $\ell$ is zero, then for each $j \in J$, we have $y_{\ell j}^\ast = 0$ thereby $\widehat{\alpha_{\ell k} y_{\ell j}} = \alpha_{\ell k}^\ast y_{\ell j}$.
%Otherwise, from \eqref{cons:material-balance-ell-approx}, we have
%\begin{equation}\label{tmp-diff-alpha}
%	\begin{aligned}
%		\alpha_{\ell k} - \alpha_{\ell k}^\ast  
%		& = 
%		\frac{
%			\sum_{i \in I} \lambda_{ik} y_{i\ell}
%			- \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j}^\ast 
%			- \alpha_{\ell k}^\ast \left(\sum_{j \in J} y_{\ell j} - \sum_{j \in J} y_{\ell j}^\ast \right) 
%		}{
%			\sum_{j \in J} y_{\ell j}^\ast
%		}\\
%		& = \frac{\sum_{i \in I} \lambda_{ik} y_{i\ell} - \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j}}{\sum_{j \in J} y_{\ell j}^\ast}.
%	\end{aligned}
%\end{equation}
%By multiplying with $y_{\ell j}^\ast$ at both left hand side and right hand side of \eqref{tmp-diff-alpha}, we obtain 
%\begin{equation*}
%	(\alpha_{\ell k} - \alpha_{\ell k}^\ast) y_{\ell j}^\ast = \frac{y_{\ell j}^\ast}{\sum_{j \in J} y_{\ell j}^\ast} \left(\sum_{i \in I} \lambda_{ik} y_{i\ell} - \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j}\right).
%\end{equation*}
%Thus, by introducing variables 
%\begin{equation}\label{def:R}
%	R_{\ell k} = \sum_{i \in I} \lambda_{i} y_{i \ell} - \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j},
%\end{equation}
%and distribution coefficients
%\begin{equation}\label{def:beta}
%	\beta_{\ell j}^\ast = \left\{
%	\begin{aligned}
%		& \frac{y_{\ell j}^\ast}{\sum_{j \in J} y_{\ell j}^\ast} && \text{ if } \sum_{j \in J} y_{\ell j}^\ast > 0;\\
%		& 0 && \text{ otherwise},
%	\end{aligned}
%	\right.
%\end{equation}
%the first order Taylor expansion $\widehat{\alpha_{\ell k} y_{\ell j}}$ can be uniformly represented as
%\begin{equation}\label{each-bilinear-betaR}
%	\widehat{\alpha_{\ell k} y_{\ell j}} = \alpha_{\ell k}^\ast y_{\ell j} + \beta_{\ell j}^\ast R_{\ell k}.
%\end{equation}
%Then by substituting the approximated bilinear terms with \eqref{each-bilinear-betaR} in equations
%\eqref{cons:material-balance-ell-approx} and inequalities \eqref{cons:material-balance-j-lb-approx}--\eqref{cons:material-balance-j-ub-approx}, we obtain
%\begin{equation}\label{cons:material-balance-ell-approx-R}
%	\sum_{i \in I} \lambda_{ik} y_{i\ell} = \alpha_{\ell k}^\ast \sum_{j \in J} y_{\ell j} + R_{\ell k} \sum_{j \in J} \beta_{\ell j}^\ast , \ \forall \ \ell \in L, \ k \in K,
%\end{equation}
%and 
%\begin{subequations}
%	\begin{align}
%		& \sum_{i \in I} \lambda_{ik} y_{ij}
%		+ \sum_{\ell \in L} 
%		\left( 
%			\alpha_{\ell k}^\ast y_{\ell j} + \beta_{\ell j}^\ast R_{\ell k}
%		\right)
%		\ge \lambda_{jk}^{\min} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K,
%		\label{cons:material-balance-j-lb-approx-R}\\
%		& \sum_{i \in I} \lambda_{ik} y_{ij}
%		+ \sum_{\ell \in L} 
%		\left( 
%			\alpha_{\ell k}^\ast y_{\ell j} + \beta_{\ell j}^\ast R_{\ell k}
%		\right) 
%		\le \lambda_{jk}^{\max} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K.
%		\label{cons:material-balance-j-ub-approx-R}
%	\end{align}
%\end{subequations}
%Therefore, problem \eqref{prob:pooling-P} can be approximated into 
%\begin{equation}\label{prob:pooling-P-approx-star}\tag{$P(y^\ast, \alpha^\ast, \beta^\ast)$}
%	\min_{y,\, R} 
%	\left\{
%	\sum_{(i,j) \in A} c_{ij} y_{ij} : 
%	\eqref{cons:flow-conservation}, 
%	\eqref{cons:material-balance-ell-approx-R}, 
%	\eqref{cons:material-balance-j-lb-approx-R}, 
%	\eqref{cons:material-balance-j-ub-approx-R}, 
%	\eqref{cons:capacity-node-i}, 
%	\eqref{cons:capacity-node-ell},
%	\eqref{cons:capacity-node-j},
%	\eqref{cons:capacity-arc}
%	\right\}.
%\end{equation}
%
%
%Next, we introduce the distributive recursion algorithm.
%% ======== Initialization ========
%To initialize, we solving a linear relaxation of problem \eqref{prob:pooling-P} with nonlinear constraints \eqref{cons:material-balance-ell}, \eqref{cons:material-balance-j-lb}, and \eqref{cons:material-balance-j-ub} and quality variables $\alpha$ dropped, obtaining an initial solution $y^0$. 
%\red{(How to define $\alpha^0$?)}
%%Besides, we take \red{$\beta^0 = ?$} and 
%% ======= How to update =======
%At each iteration $t + 1$ ($t \ge 0$), we first compute $\alpha^{t}$ and $\beta^{t}$ with $y^{t}$, which has been calculated at the $(t-1)$-th iteration.
%For each $\ell \in L$, 
%\begin{itemize}
%	\item if $\sum_{j \in J} y_{\ell j}^{t} = 0$, let \red{$\alpha_{\ell k}^{t} = \alpha_{\ell k}^{t-1}$} for $k \in K$ and \red{$\beta_{\ell j}^{t} = 0$} for $j \in J$.
%	\item otherwise, let $\alpha_{\ell k}^{t} = \sum_{i \in I} \lambda_{ik} y_{i \ell}^{t} / \sum_{j \in J} y_{\ell j}^{t}$ for $k \in K$ and $\beta_{\ell j}^{t} = y_{i \ell}^{t} / \sum_{j \in J} y_{\ell j}^{t}$ for $j \in J$.
%\end{itemize}
%Then we solve problem \ref{prob:pooling-P-approx-star} by substituting $\alpha^\ast$, $y^\ast$, and $\beta^\ast$ with $\alpha^{t}$, $y^{t}$, and $\beta^{t}$, respectively.
%Given an initial solution $(y^0, \alpha^0)$, the acceptance $\epsilon$ and maximal number of iteration $t_{\max}$, 
%summarize the \DR approach in \cref{alg:DR}
%\begin{algorithm}[htbp]
%	\caption{Distributed\_Recursion($y^0, \alpha^0, \epsilon$, $t_{\max}$)}
%	\label{alg:DR}
%	\ForEach{$t = 0, 1, \dots, t_{\max} - 1$}{
%		\ForEach{$\ell \in L$}{
%			\eIf{$\sum_{j \in J} y_{\ell j}^t = 0$}{
%				\If{$t \ge 1$}{
%				\lForEach{$k \in K$}{$\alpha_{\ell k}^t \leftarrow \alpha_{\ell k}^{t-1}$}}
%				\lForEach{$j \in J$}{$\beta_{\ell j}^t \leftarrow 0$}
%			}{
%				\lForEach{$k \in K$}{$\alpha_{\ell k}^{t} \leftarrow \sum_{i \in I} \lambda_{ik} y_{i \ell}^{t} / \sum_{j \in J} y_{\ell j}^{t}$}
%				\lForEach{$j \in J$}{$\beta_{\ell j}^{t} \leftarrow y_{i \ell}^{t} / \sum_{j \in J} y_{\ell j}^{t}$}
%			}
%		}
%		$(y^{t+1}, R^{t+1}) \leftarrow$ Solve \ref{prob:pooling-P-approx-star} where $y^\ast = y^{t}$, $\alpha^\ast = \alpha^{t}$, and $\beta^\ast = \beta^{t}$\;
%		\lIf{$\max_{\ell \in L, \ k \in K} |R_{\ell k}| < \epsilon$}{\textbf{break}}
%	}
%	\KwRet{$y^{t+1}, \alpha^{t+1}$}
%\end{algorithm}
%
\subsection{Equivalence between the \DR approach and the \SLP}

\begin{lemma}\label{lem:approx-bilinear-equiv}
	\red{Given $y^\ast$ (add more restrictions for $y^\ast$)}, let $L_0(y^\ast)$ be defined as in \eqref{def:L0} and $\alpha^\ast$ be such that equations \eqref{cons:material-balance-ell} hold for all $\ell \in L \backslash L_0(y^\ast)$ and $k \in K$.
	Moreover, let $\beta^\ast$ be defined by \eqref{def:beta}, respectively.
	Then equation
	\begin{equation}\label{tmp-approx-equiv0}
		\alpha^\ast_{\ell k} y_{\ell j}^\ast +	 \alpha^\ast_{\ell k}(y_{\ell j} - y_{\ell j}^\ast) = \alpha_{\ell k}^\ast y_{\ell j} + \beta^\ast_{\ell j} \left( 
		\sum_{i' \in I} \lambda_{i'k} y_{i' \ell}
		- \sum_{j' \in J} \alpha_{\ell k}^\ast y_{\ell j'}
		\right)
	\end{equation}
	holds for $\ell \in L_0(y^\ast)$, $k \in K$, and $j \in J$, and equation 
	\begin{equation}\label{tmp-approx-equiv1}
		\begin{aligned}
			& F_{\ell k}(y^\ast; \alpha^\ast) y_{\ell j}^\ast + \sum_{(i',j') \in A} \frac{\partial (F_{\ell k}(y^\ast; \alpha^\ast) y_{\ell j}^\ast)}{\partial y_{i' j'}} (y_{i' j'} - y_{i' j'}^\ast) \\
			& \qquad \qquad = \alpha_{\ell k}^\ast y_{\ell j} + \beta^\ast_{\ell j} \left( 
			\sum_{i' \in I} \lambda_{i'k} y_{i' \ell}
			- \sum_{j' \in J} \alpha_{\ell k}^\ast y_{\ell j'}
			\right)
		\end{aligned}
	\end{equation}
	holds for $\ell \in L \backslash L_0(y^\ast)$, $k \in K$, and $j \in J$.
\end{lemma}
\begin{proof}
	Let $\ell \in L$, $k \in K$, and $j \in J$.
	If $\ell \in L_0(y^\ast)$, then from the definition of $L_0(y^\ast)$ \eqref{def:L0}, $y_{\ell j}^\ast = 0$ holds thereby $\alpha^\ast_{\ell k}(y_{\ell j} - y_{\ell j}^\ast) = \alpha^\ast_{\ell k} y_{\ell j}$.
	From $\ell \in L_0(y^\ast)$ and the definitions of $L_0(y^\ast)$ \eqref{def:L0} and $\beta^\ast$ \eqref{def:beta}, we have $\beta_{\ell j}^\ast  =0$ thereby $\alpha_{\ell k}^\ast y_{\ell j} + \beta^\ast_{\ell j} R_{\ell k} = \alpha_{\ell k}^\ast y_{\ell j}$.
	Thus \eqref{tmp-approx-equiv0} holds.
	If $\ell \in L \backslash L_0(y^\ast)$, then from the definition of $\alpha^\ast$, we have
	\begin{equation}\label{tmp-alpha}
		\alpha_{\ell k}^\ast = \frac{\sum_{i'' \in I} \lambda_{i'' k} y_{i'' \ell}^\ast}{ \sum_{j'' \in J} y_{\ell j''}^\ast}= F_{\ell k}(y^\ast; \alpha^\ast).
	\end{equation}
	From the definition of $F_{\ell k}$ \eqref{def:func-f}, 
	for each $(i',j') \in A$, we have 
	\begin{equation}\label{tmp-derivative-F}
		\frac{\partial F_{\ell k}(y^\ast; \alpha^\ast_{\ell k})}{\partial y_{i' j'}} = 
		\left\{ \ 
		\begin{aligned}
			& \frac{\lambda_{i'k}}{\sum_{j'' \in J} y_{\ell j}^\ast},
			&& \text{ if } i' \in I \text{ and } j' = \ell; \\
			& - \frac{\sum_{i'' \in I} \lambda_{i'' k} y_{i'' \ell}^\ast}{\left(\sum_{j'' \in J} y_{\ell j''}^\ast\right)^2},
			&& \text{ if } j' \in J \text{ and } i' = \ell; \\
			& 0, 
			&& \text{ otherwise},
		\end{aligned}
		\right. \quad \forall \ (i', j') \in A.
	\end{equation}
	Thus we have
	\begin{equation*}
		\begin{aligned}
			& F_{\ell k}(y^\ast; \alpha^\ast) y^\ast_{\ell j} + \sum_{(i',j') \in A} \frac{\partial (F_{\ell k}(y^\ast; \alpha^\ast_{\ell k}) y_{\ell j}^\ast)}{\partial y_{i' j'}} (y_{i' j'} - y_{i' j'}^\ast)\\
			& \quad = F_{\ell k}(y^\ast; \alpha^\ast) y^\ast_{\ell j} + \sum_{(i',j') \in A} \left(\frac{\partial F_{\ell k}(y^\ast; \alpha^\ast_{\ell k})}{\partial y_{i' j'}} y_{\ell j}^\ast + 
			\frac{\partial y_{\ell j}^\ast}{\partial y_{i' j'}} F_{\ell k}(y^\ast; \alpha^\ast_{\ell k})\right)(y_{i' j'} - y_{i' j'}^\ast)\\
			& \quad \overset{\text{(a)}}{=} F_{\ell k}(y^\ast; \alpha^\ast) y^\ast_{\ell j} + 
			\sum_{(i',j') \in (I \times \{\ell\}) \cup (\{\ell\} \times J)} \frac{\partial F_{\ell k}(y^\ast; \alpha^\ast_{\ell k})}{\partial y_{i' j'}} y_{\ell j}^\ast (y_{i' j'} - y_{i' j'}^\ast)
			+ F_{\ell k}(y^\ast; \alpha^\ast) (y_{\ell j} - y_{\ell j}^\ast)\\
			& \quad \overset{\text{(b)}}{=}
			\sum_{i \in I} \frac{\lambda_{i'k}}{\sum_{j'' \in J} y_{\ell j}^\ast} 
			y_{\ell j}^\ast (y_{i' \ell} - y_{i' \ell}^\ast)
			- \sum_{j' \in J} \frac{\sum_{i'' \in I} \lambda_{i'' k} y_{i'' \ell}^\ast}{\left(\sum_{j'' \in J} y_{\ell j''}^\ast\right)^2}
			y_{\ell j}^\ast (y_{\ell j'} - y_{\ell j'}^\ast)
			+ F_{\ell k}(y^\ast; \alpha^\ast) y_{\ell j}\\
			& \quad \overset{\text{(c)}}{=}
			\sum_{i' \in I} \frac{\lambda_{i'k}}{\sum_{j'' \in J} y_{\ell j}^\ast} 
			y_{\ell j}^\ast (y_{i' \ell} - y_{i' \ell}^\ast)
			- \sum_{j' \in J} \frac{\alpha_{\ell k}^\ast}{\sum_{j'' \in J} y_{\ell j''}^\ast}
			y_{\ell j}^\ast (y_{\ell j'} - y_{\ell j'}^\ast)
			+ \alpha_{\ell k}^\ast y_{\ell j}\\
			& \quad = \frac{y_{\ell j}^\ast}{\sum_{j'' \in J} y_{\ell j''}^\ast}
			\left( 
				\sum_{i' \in I} \lambda_{i'k} (y_{i' \ell} - y_{i' \ell}^\ast)
				- \sum_{j' \in J} \alpha_{\ell k}^\ast (y_{\ell j'} - y_{\ell j'}^\ast)
			\right)
			+ \alpha_{\ell k}^\ast y_{\ell j}\\
			& \quad \overset{\text{(d)}}{=} \frac{y_{\ell j}^\ast}{\sum_{j'' \in J} y_{\ell j''}^\ast}
			\left( 
			\sum_{i' \in I} \lambda_{i'k} y_{i' \ell}
			- \sum_{j' \in J} \alpha_{\ell k}^\ast y_{\ell j'}
			\right)
			+ \alpha_{\ell k}^\ast y_{\ell j}\\
			& \quad \overset{\text{(e)}}{=} \beta_{\ell j}^\ast \left( 
			\sum_{i' \in I} \lambda_{i'k} y_{i' \ell}
			- \sum_{j' \in J} \alpha_{\ell k}^\ast y_{\ell j'}
			\right)
			+ \alpha_{\ell k}^\ast y_{\ell j}\\
		\end{aligned}
	\end{equation*}
	where (a) follows as $\frac{\partial F_{\ell k}(y^\ast; \alpha^\ast)}{\partial y^{i' j'}} = 0$ if $(i',j') \notin (I \times \{\ell\}) \cup (\{\ell\} \times J)$ and $\frac{\partial y_{\ell j}^\ast}{y_{i'j'}} = 0$ if $(i',j') \neq (\ell, j)$; (b) follows from \eqref{tmp-derivative-F}; (c) follows from \eqref{tmp-alpha}; (d) follows from the fact that equations \eqref{cons:material-balance-ell} where $\ell \in L \backslash L_0(y^\ast)$ and $k \in K$ hold at point $(y^\ast,\alpha^\ast)$; and (e) follows from the definition of $\beta^\ast$.
	Thus \eqref{tmp-approx-equiv1} holds.
\end{proof}

Given $y^\ast$, let $L_0(y^\ast)$, $\alpha^\ast$, and $\beta^\ast$ be defined as in \cref{lem:approx-bilinear-equiv}.
Then linear systems $\{\eqref{cons:material-balance-j-lb-Fy-linear0}, \eqref{cons:material-balance-j-ub-Fy-linear0}\}$ and $\{\eqref{cons:material-balance-ell-approx-R}, \eqref{cons:material-balance-j-lb-approx-R}, \eqref{cons:material-balance-j-ub-approx-R}\}$ are equivalent.
Therefore, we have the following result.
\begin{theorem}
	Given $(\alpha^0, y^0)$ satisfying equations \eqref{cons:material-balance-ell}, we initialize both the \SLP and \DR with $(\alpha^0, y^0)$.
	Denote $y^{t,\SLP}$ and $(y^{t,\DR}, R^{t, \DR})$ as the solutions of $t$-th iteration of the \SLP and \DR, respectively, for $t = 1, \dots, t_{\max}$.
	If $y^{t', \SLP} = y^{t', \DR}$ for $t' = 1, \dots, t-1$, then at $t$-th iteration problem \eqref{prob:pooling-P-y-star} is the projection of \eqref{prob:pooling-P-approx-star} in the $y$-variable space.
\end{theorem}



%prove that at each iteration, the linear programming problem \eqref{prob:pooling-Y-SLP} defined by $(\alpha^t, y^t)$ and \eqref{prob:pooling-P-DR} defined by the same are equivalent.
%
%In this section, we give the relationship between the constraints \eqref{cons:material-balance-j-lb-y}, \eqref{cons:material-balance-j-ub-y} generated by SLP method and the constraints \eqref{cons:material-balance-j-all-linear} generated by DR method. We assume that $k\equiv1$ for abbreviation and set $\alpha_\ell:=\alpha_{\ell k}$, $\lambda_i:=\lambda_{ik}$, $R_{\ell k}:=R_{\ell k}$, $F_{\ell}(y):=F_{\ell k}(y)$.
%
%Substitute $R_\ell$ from \eqref{cons:material-balance-ell-layer-linear} into the second term of \eqref{cons:material-balance-j-all-linear}, we derive that
%\begin{align*}
%	&\quad\alpha_{\ell}^ty_{\ell j}+\beta_{\ell j}^tR_{\ell k}\\
%	&=\alpha_{\ell}^ty_{\ell j}+\beta_{\ell j}^t\left(\sum_{i\in I}\lambda_{i}y_{i\ell}-\alpha_\ell^t\sum_{j\in J}y_{\ell j}\right)\\
%	&=\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}y_{\ell j}+\frac{y_{\ell j}^t}{\sum_{j\in J}y_{\ell j}^t}\left(\sum_{i\in I}\lambda_{i}y_{i\ell}-\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}\sum_{j\in J}y_{\ell j}\right)\\
%	&=\frac{1}{\sum_{j\in J}y_{\ell j}^t}\left(y_{\ell j}\sum_{i\in I}\lambda_iy_{i\ell}^t + y_{\ell j}^t\sum_{i\in I}\lambda_{i}y_{i\ell}\right) -\frac{y_{\ell j}^t}{\sum_{j\in J}y_{\ell j}^t}\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}\sum_{j\in J}y_{\ell j}\\
%	&=\frac{y_{\ell j}\sum_{i\in I}\lambda_iy_{i\ell}^t + y_{\ell j}^t\sum_{i\in I}\lambda_{i}y_{i\ell} - \frac{\sum_{j\in J}y_{\ell j}}{\sum_{j\in J}y_{\ell j}^t}y_{\ell j}^t\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}, \quad \ell\in L^t.
%\end{align*}
%For all $\ell\in L^t, j\in J$, we define that
%\begin{equation}\label{eq18}
%h_{\ell j}(y,y^t):=\frac{y_{\ell j}\sum_{i\in I}\lambda_iy_{i\ell}^t + y_{\ell j}^t\sum_{i\in I}\lambda_{i}y_{i\ell} - \frac{\sum_{j\in J}y_{\ell j}}{\sum_{j\in J}y_{\ell j}^t}y_{\ell j}^t\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}.
%\end{equation}
%Moreover, for $\ell\in L$ such that $\sum_{j \in  J} y_{\ell j}^t=0$, it follows from \eqref{alpha_renew} and \eqref{beta_renew} that
%\begin{equation}\label{hlj}
%h_{\ell j}(y,y^t):=\alpha_{\ell}^ty_{\ell j}+\beta_{\ell j}^tR_{\ell k}=\alpha_{\ell}^{t-1}y_{\ell j}.
%\end{equation}
%
%We reform the DR subproblem \eqref{prob:pooling-P-DR} as
%\begin{align*}
%	\max_{y,R} \quad &\sum_{j\in J}c_{j}\sum_{\ell\in I\cup L}y_{\ell j}-\sum_{i\in I}c_{i}\sum_{\ell\in L\cup J}y_{i\ell} \\
%	\mathrm{s.~t.}
%	&\sum_{i\in I}\lambda_{i}y_{ij}+\sum_{\ell\in L^t}h_{\ell j}(y,y^t)\geq\lambda_j^{\min}\sum_{i\in I\cup L}y_{ij},\forall j\in J,\label{eq1.13}\\
%	&\sum_{i\in I}\lambda_{i}y_{ij}+\sum_{\ell\in L^t}h_{\ell j}(y,y^t)\leq\lambda_j^{\max}\sum_{i\in I\cup L}y_{ij},\forall j\in J,\\
%	&
%	\eqref{cons:flow-conservation},
%	\eqref{cons:capacity-node-i},
%	\eqref{cons:capacity-node-ell},
%	\eqref{cons:capacity-node-j},
%	\eqref{cons:capacity-arc}.\nonumber
%\end{align*}
%
%
%


%\begin{lemma}\label{lem5.1}
%Given two constant vectors $\lambda\in\mathbb{R}^n$, $e\in\mathbb{R}^n$ and a variable vector $y\in\mathbb{R}^n$, define two functions
%\begin{equation}\label{eq19}
%\hat h(y,y^t):=\frac{y\lambda^Ty^t+y^t\lambda^Ty-\frac{e^Ty}{e^Ty^t}y^t\lambda^Ty^t}{e^Ty^t},
%\quad 
%\hat f(y):=\frac{y\lambda^Ty}{e^Ty}.
%\end{equation}
%If $e^Ty^t\ne0$, then
%\[
%\hat h(y,y^t)=\hat f(y^t)+\frac{\partial \hat f(y^t)}{\partial y}(y-y^t).
%\]
%%$\hat h(y,y^t)-\hat f(y)=O(\|y-y^t\|^2)$.
%\end{lemma}
%
%\begin{proof}
%By the assumption $e^Ty^t\ne0$, the defined function $\hat f(y)$ is twice continuously differentiable at $y^t$. Therefore, it holds for $y$ sufficiently close to $y^t$ that
%\[
%\frac{\partial \hat f(y)}{\partial y}=\frac{e^Ty(\lambda^TyI+y\lambda^T)-y\lambda^Tye^T}{(e^Ty)^2}.
%\]
%Hence, we derive that
%\begin{align*}
%	\hat f(y^t)+\nabla \hat f(y^t)^T(y-y^t)
%	&=\frac{y^t\lambda^Ty^t}{e^Ty^t}+\frac{e^Ty^t(\lambda^Ty^tI+y^t\lambda^T)-y^t\lambda^Ty^te^T}{(e^Ty^t)^2}(y-y^t)\\
%	&=\frac{y^t\lambda^Ty^t+(\lambda^Ty^tI+y^t\lambda^T)(y-y^t)-\frac{y^t\lambda^Ty^te^T(y-y^t)}{e^Ty^t}}{e^Ty^t}\\
%	&=\frac{y\lambda^Ty^t+y^t\lambda^Ty-y^t\lambda^Ty^t-\frac{y^t\lambda^Ty^te^Ty-y^t\lambda^Ty^te^Ty^t}{e^Ty^t}}{e^Ty^t}\\
%	&=\frac{y\lambda^Ty^t+y^t\lambda^Ty-\frac{e^Ty}{e^Ty^t}y^t\lambda^Ty^t-y^t\lambda^Ty^t+y^t\lambda^Ty^t}{e^Ty^t}\\
%	&=\frac{y\lambda^Ty^t+y^t\lambda^Ty-\frac{e^Ty}{e^Ty^t}y^t\lambda^Ty^t}{e^Ty^t}\\
%	&=\hat h(y,y^t).
%\end{align*}
%The proof is completed.
%\end{proof}
%
%\subsection{Error bounds}
%\begin{Theorem}
%	The error between $h_{\ell j}(y,y^t)$ and $f_{\ell j}(y)$ $(\forall \ell\in L, j\in J)$satisfies that
%	\[
%	h_{\ell j}(y,y^t) - f_{\ell j}(y) = O(\|y-y^t\|^2).
%	\]
%\end{Theorem}
%
%\begin{proof}
%	Since both $\sum_{i\in I}\lambda_{i}y_{i\ell}$ and $\sum_{j\in J}y_{\ell j}^t$ are determined linearly with respect to $y_{\ell j}$, there exists two vector $(\lambda,e)$ with suitable dimensions such that
%	\[
%	\sum_{i\in I}\lambda_{i}y_{i\ell}=\lambda^Ty, \quad \sum_{j\in J}y_{\ell j}=e^Ty,
%	\]
%	where $y$ is a variable extracted from $\{y_{\ell j}\}$. Moreover, we set similarly that $\sum_{i\in I}\lambda_{i}y_{i\ell}^t=\lambda^Ty^t$ and $\sum_{j\in J}y_{\ell j}^t=e^Ty^t$. Then, according to \eqref{eq18} and \eqref{eq19}, we have
%	\begin{equation}\label{eq20}
%	h_{\ell j}(y,y^t)=\hat h_{\ell j}(y,y^t), \quad f_{\ell j}(y)=\hat f_{\ell j}(y).
%	\end{equation}
%	The rest proof follows directly from Lemma \ref{lem5.1}, \eqref{eq20} and the first-order Taylor expansion
%	\[
%	f_{\ell j}(y)=f_{\ell j}(y^t)+\frac{\partial f_{\ell j}(y^t)}{\partial y}(y-y^t)+O(\|y-y^t\|^2).
%	\]
%\end{proof}

% ================================

%\begin{align*}
%	\alpha^t_{\ell} y_{\ell j} + \beta^t_{\ell j} R_{\ell k}
%	& = h_{\ell j}(y, y^t)
%\end{align*}
%
%\begin{align*}
%	&\quad\alpha_{\ell}^ty_{\ell j}+\beta_{\ell j}^tR_{\ell k}\\
%	&=\alpha_{\ell}^ty_{\ell j}+\beta_{\ell j}^t\left(\sum_{i\in I}\lambda_{i}y_{i\ell}-\alpha_\ell^t\sum_{j\in J}y_{\ell j}\right)\\
%	&=\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}y_{\ell j}+\frac{y_{\ell j}^t}{\sum_{j\in J}y_{\ell j}^t}\left(\sum_{i\in I}\lambda_{i}y_{i\ell}-\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}\sum_{j\in J}y_{\ell j}\right)\\
%	&=\frac{1}{\sum_{j\in J}y_{\ell j}^t}\left(y_{\ell j}\sum_{i\in I}\lambda_iy_{i\ell}^t + y_{\ell j}^t\sum_{i\in I}\lambda_{i}y_{i\ell}\right) -\frac{y_{\ell j}^t}{\sum_{j\in J}y_{\ell j}^t}\frac{\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}\sum_{j\in J}y_{\ell j}\\
%	&=\frac{y_{\ell j}\sum_{i\in I}\lambda_iy_{i\ell}^t + y_{\ell j}^t\sum_{i\in I}\lambda_{i}y_{i\ell} - \frac{\sum_{j\in J}y_{\ell j}}{\sum_{j\in J}y_{\ell j}^t}y_{\ell j}^t\sum_{i\in I}\lambda_iy_{i\ell}^t}{\sum_{j\in J}y_{\ell j}^t}, \quad \ell\in L^t.
%\end{align*}


%\begin{theorem}
%At $t$-th iteration, we have
%\[
%F_{\ell}(y)y_{\ell j} + \frac{\partial(F_{\ell}(y^t)y_{\ell j}^t)}{\partial y}(y-y^t) = h_{\ell j}(y,y^t).
%\]
%\end{theorem}
%
%\begin{proof}
%We define for abbreviation that $c_{\ell j}(y):=F_{\ell}(y)y_{\ell j}$, $(\ell,j)\in L^t\times J$, then
%\begin{equation}\label{eq19}
%	c_{\ell j}(y)=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}}{\sum_{j \in J}y_{\ell j}}y_{\ell j}.
%\end{equation}
%For $\ell\in L$ such that $\sum_{j \in  J} y_{\ell j}^t=0$, we have
%\[
%c_{\ell j}(y^t)=0,
%\]
%\begin{align*}
%\nabla c_{\ell j}(y^t)^T(y-y^t)
%&=y_{\ell j}^t\nabla F_{\ell}(y^t)^T(y-y^t)+F_{\ell}(y^t)(\nabla y_{\ell j}^t)^T(y-y^t)\\
%&=F_{\ell}(y^t)(y_{\ell j}-y_{\ell j}^t)\\
%&=F_{\ell}(y^t)y_{\ell j}.
%\end{align*}
%Therefore, the proof follows by \eqref{eq8} and \eqref{hlj}.
%For $\ell\in L^t:=\{\ell\in L|\sum_{j \in  J} y_{\ell j}^t>0\}$, $j\in J$, 
%it remains to proof that
%\[
%c_{\ell j}(y^t)+\frac{\partial c_{\ell j}(y^t)}{\partial y}(y-y^t)=h_{\ell j}(y,y^t).
%\]
%We divide the index set $\{(\ell_1,\ell_2)\}$ into four separated sets:
%\[
%\{(\ell_1,\ell_2)\in I\times L\}, \quad \{(\ell_1,\ell_2)\in I\times J\}, \quad \{(\ell_1,\ell_2)\in L^t\times J\}, \quad \{(\ell_1,\ell_2)\in(L\setminus L^t)\times J\},
%\]
%and consider the derivatives of $c_{\ell j}(y)$ with respect to $y_{\ell_1\ell_2}$.
%
%Case 1: For $(\ell_1,\ell_2)\in I\times L$, we have
%\begin{equation}\label{eq20}
%\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1\ell_2}}=
%\left\{\begin{aligned}
%	&\frac{\lambda_{\ell_1}}{\sum_{j \in J}y_{\ell j}}y_{\ell j}, & \text{~if~}\ell_2=\ell; \\
%	&0, & \text{~if~}\ell_2\ne\ell.
%\end{aligned}\right.
%\end{equation}
%
%Case 2: For $(\ell_1,\ell_2)\in I\times J$, we have
%\begin{equation}\label{eq21}
%\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1\ell_2}}=0,
%\end{equation}
%
%Case 3.1: For $(\ell_1,\ell_2)\in L^t\times J$, if $(\ell_1,\ell_2)=(\ell,j)$, then
%\begin{equation}\label{eq22}
%	\begin{aligned}
%	\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1\ell_2}}
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}}{\sum_{j \in J}y_{\ell j}}+\frac{\partial(\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}}{\sum_{j \in J}y_{\ell j}})}{\partial y_{\ell j}}y_{\ell j}\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}}{\sum_{j \in J}y_{\ell j}}+\frac{\partial(\frac{1}{\sum_{j \in J}y_{\ell j}})}{\partial y_{\ell j}}(\sum_{i \in I} \lambda_{i} y_{i\ell})y_{\ell j}\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}}{\sum_{j \in J}y_{\ell j}}-\frac{1}{(\sum_{j \in J}y_{\ell j})^2}(\sum_{i \in I} \lambda_{i} y_{i\ell})y_{\ell j}.
%\end{aligned}
%\end{equation}
%
%Case 3.2: For $(\ell_1,\ell_2)\in L^t\times J$, if $\ell_1=\ell$ but $\ell_2\ne j$, then
%\begin{equation}\label{eq23}
%	\begin{aligned}
%	\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1\ell_2}}
%	=\frac{\partial\frac{1}{\sum_{j \in J}y_{\ell j}}}{\partial y_{\ell_1\ell_2}}(\sum_{i \in I} \lambda_{i} y_{i\ell})y_{\ell j}
%	=-\frac{1}{\sum_{j \in J}(y_{\ell j})^2}(\sum_{i \in I} \lambda_{i} y_{i\ell})y_{\ell j}.
%\end{aligned}
%\end{equation}
%
%Case 3.3: For $(\ell_1,\ell_2)\in L^t\times J$, if $\ell_1\ne\ell$, then
%\begin{equation}\label{eq24}
%\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1,\ell_2}}=0.
%\end{equation}
%
%Case 4: For $(\ell_1,\ell_2)\in (L\setminus L^t)\times J$, we have
%\begin{equation}\label{eq26}
%	\frac{\partial c_{\ell j}(y)}{\partial y_{\ell_1\ell_2}}=0,
%\end{equation}
%
%According to 
%\[
%\frac{\partial c_{\ell j}(y)}{\partial y}(y-y^t)=\sum_{\ell_1,\ell_2}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)
%\]
%equation \eqref{eq21} and \eqref{eq26}, we have
%\begin{equation}\label{eq28}
%\begin{aligned}
%\frac{\partial c_{\ell j}(y)}{\partial y}(y-y^t)
%=\sum_{(\ell_1,\ell_2)\in I\times L}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)
%+\sum_{(\ell_1,\ell_2)\in L^t\times J}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t).
%\end{aligned}
%\end{equation}
%To be more precisely, for the second term in \eqref{eq28}, it holds that
%\begin{equation}\label{eq25}
%	\begin{aligned}
%	\sum_{(\ell_1,\ell_2)\in I\times L}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)
%	&\overset{\eqref{eq20}}{=}\sum_{\ell_1\in I,\ell_2=\ell}\frac{\lambda_{\ell_1}}{\sum_{j \in J}y_{\ell j}}y_{\ell j}^t(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)\\
%	&=\frac{\sum_{\ell_1\in I}\lambda_{\ell_1}(y_{\ell_1\ell}-y_{\ell_1\ell}^t)}{\sum_{j \in J}y_{\ell j}^t}y_{\ell j}^t\\
%	&=\frac{\sum_{i\in I}\lambda_{i}y_{i\ell}y_{\ell j}^t-\sum_{i\in I}\lambda_{i}y_{i\ell}^ty_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t},
%\end{aligned}
%\end{equation}
%and for the third term in \eqref{eq28}, there is
%\begin{equation}\label{eq27}
%\begin{aligned}
%	&\quad\sum_{(\ell_1,\ell_2)\in L^t\times J}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)\\
%	&\overset{\eqref{eq22}-\eqref{eq24}}{=}\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^t}{\sum_{j \in J}y_{\ell j}^t}(y_{\ell j}-y_{\ell j}^t)
%	+\sum_{\ell_1=\ell,\ell_2\in J}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^t}{\sum_{j \in J}y_{\ell j}^t}(y_{\ell j}-y_{\ell j}^t)
%	-\sum_{\ell_1=\ell,\ell_2\in J}\frac{1}{\sum_{j \in J}(y_{\ell j}^t)^2}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^t}{\sum_{j \in J}y_{\ell j}^t}(y_{\ell j}-y_{\ell j}^t)
%	-\frac{\sum_{\ell_1=\ell,\ell_2\in J}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)}{\sum_{j \in J}(y_{\ell j}^t)^2}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^t}{\sum_{j \in J}y_{\ell j}^t}(y_{\ell j}-y_{\ell j}^t)
%	-\frac{\sum_{j\in J}y_{\ell j}-\sum_{j\in J}y_{\ell j}^t}{\sum_{j \in J}(y_{\ell j}^t)^2}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^t(y_{\ell j}-y_{\ell j}^t)-\frac{\sum_{j\in J}y_{\ell j}}{\sum_{j \in J}y_{\ell j}^t}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t+(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t}\\
%	&=\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^ty_{\ell j}-\frac{\sum_{j\in J}y_{\ell j}}{\sum_{j \in J}y_{\ell j}^t}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t}.
%\end{aligned}
%\end{equation}
%Combine \eqref{eq28}-\eqref{eq27} together, we deduce that
%\begin{equation}\label{eq29}
%	\begin{aligned}
%	&\quad\frac{\partial c_{\ell j}(y^t)}{\partial y}(y-y^t)\\
%%	&=\sum_{\ell_1,\ell_2}\frac{\partial c_{\ell j}(y^t)}{\partial y_{\ell_1\ell_2}}(y_{\ell_1\ell_2}-y_{\ell_1\ell_2}^t)\\
%	&=\frac{\sum_{i\in I}\lambda_{i}y_{i\ell}y_{\ell j}^t-\sum_{i\in I}\lambda_{i}y_{i\ell}^ty_{\ell j}^t+\sum_{i \in I} \lambda_{i} y_{i\ell}^ty_{\ell j}-\frac{\sum_{j\in J}y_{\ell j}}{\sum_{j \in J}y_{\ell j}^t}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t}.
%\end{aligned}
%\end{equation}
%Therefore,
%\begin{align*}
%	 c_{\ell j}(y^t)+\frac{\partial c_{\ell j}(y^t)}{\partial y}(y-y^t)
%	&\overset{\eqref{eq19}}{=}\frac{\sum_{i \in I} \lambda_{i} y_{i\ell}^ty_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t}+\frac{\partial c_{\ell j}(y^t)}{\partial y}(y-y^t)\\
%	&\overset{\eqref{eq29}}{=}\frac{\sum_{i\in I}\lambda_{i}y_{i\ell}y_{\ell j}^t+\sum_{i \in I} \lambda_{i} y_{i\ell}^ty_{\ell j}-\frac{\sum_{j\in J}y_{\ell j}}{\sum_{j \in J}y_{\ell j}^t}(\sum_{i \in I} \lambda_{i} y_{i\ell}^t)y_{\ell j}^t}{\sum_{j \in J}y_{\ell j}^t}\\
%	&\overset{\eqref{eq18}}{=}h_{\ell j}(y,y^t).
%\end{align*}
%The proof is completed.
%\end{proof}









% ====================================================











%In this section, we will show that the newly proposed formulation \eqref{prob:pooling-P-y} admits the use of the successive linear programming (\SLP, \citet{Baker1985,Zhang1985}) approach.
%In this section, we first present the solution approach of distributed recursion (\DR, \citet{Haverly1978,Haverly1979,Haverly1980}) for problem  \eqref{prob:pooling-P}.
%Then we show the equivalence of \DR on \eqref{prob:pooling-P} and \SLP on \eqref{prob:pooling-P-y}, which provides a novel and rigorous interpretation for the distributed recursion approach. 
%\todo[inline]{In this section, we provide the distributed recursion (\DR, \citet{Haverly1978,Haverly1979,Haverly1980}) approach for problem \eqref{prob:pooling-P} and demonstrate the equivalence of \DR on \eqref{prob:pooling-P} and \SLP on \eqref{prob:pooling-P-y}.}
%In the following subsection, 


%\subsection{Distributed recursion approach for solving \eqref{prob:pooling-P}} \label{subsect:DR}
%we consider the properties at the outputs to be within specified bounds \eqref{cons:material-balance-j-lb} and \eqref{cons:material-balance-j-ub}:
%	\begin{subequations}\label{cons:material-balance-j-all} 
	%		\begin{align}
		%		& \sum_{i \in I} \lambda_{ik} y_{ij}
		%		+ \sum_{\ell \in L} \alpha_{\ell k} y_{\ell j} \ge \lambda_{jk}^{\min} \sum_{i \in I \cup L} y_{ij},\ \forall \ j \in J, \ k \in K,\\
		%		& \sum_{i \in I} \lambda_{ik} y_{ij}
		%		+ \sum_{\ell \in L} \alpha_{\ell k} y_{\ell j} \le 	\lambda_{jk}^{\max} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K.
		% \end{align}\end{subequations}
%	For every $\alpha_{\ell k} y_{\ell j}$, it comes from  the pools, and the pools satisfy the balance constraint \eqref{cons:material-balance-ell}:
%	\begin{equation}\label{cons:material-balance-ell-layer}
	%		\sum_{i \in I} \lambda_{ik} y_{i\ell} 
	%		= \alpha_{\ell k} \sum_{j \in J} y_{\ell j}, \ \forall \ \ell \in L, k \in K. 
	%	\end{equation}


%	Because there exist nonlinear terms $\alpha_{\ell k}y_{\ell j}$,   \eqref{prob:pooling-P} is hard to solve, so we want to solve it as an LP model. In the pooling problem, a method has been widely applied, DR. It integrates the error between predicted and computed values into the model. For each recursive specification variable in the model, an error variable is defined, representing the discrepancy between the predicted specification and the calculated value. This error is then distributed to subsequent nodes according to the  direction and the corresponding proportionality coefficients of the flow. That is, for the nonlinear term $\alpha_{\ell k}y_{\ell j}$, given $\alpha_{\ell k}^t$, we have the linear term:
%	\begin{equation}\label{tmpeq}
	%		\alpha_{\ell k}^ty_{\ell j} + \beta_{\ell j}^tR_{\ell k},
	%	\end{equation} 
%	here,  $\beta_{\ell j}^t$ is the corresponding proportionality coefficients about the pool $\ell$ flow to output $j$, $R_{\ell k}$ is the 
%	error variable.
%\todo[inline]{YW: Do we need to present the above red paragraphs?\\
	%WZ: we need this, it is the DR method in industry}
%
%For brevity of notations, we drop the subscripts $k$.
%It is known that the first order Taylor polynomial of $g(x_1, x_2)$ at point $(\bar{x}_1, \bar{x}_2)$ is 
%\begin{equation*}
%	P_1(x^1, x^2) = g(\bar{x}_1, \bar{x}_2) + g_{x_1}(\bar{x}_1, \bar{x}_2)(x_1 - \bar{x}_1) + g_{x_2}(\bar{x}_1, \bar{x}_2)(x_2 - \bar{x}_2).
%\end{equation*}
%%https://math.libretexts.org/Bookshelves/Calculus/Calculus_3e_(Apex)/08%3A_Sequences_and_Series/8.07%3A_Taylor_Polynomials
%%https://www.math.ucla.edu/~tsmits/Teaching/32A/Handouts/TaylorPoly.pdf
%Then for each $j$, we can obtain the first order Taylor polynomial of $\alpha_{\ell} y_{\ell j} = g(\alpha_{\ell}, y_{\ell j})$ at point $(\alpha_{\ell}^t, y_{\ell j}^t)$:
%\begin{equation}\label{1st-Taylor}
%	\begin{aligned}
	%		\widehat{\alpha_{\ell} y_{\ell j}} = & \alpha_{\ell}^t y_{\ell j}^t + y_{\ell j}^t (\alpha_{\ell} - \alpha_{\ell}^t) + \alpha_{\ell}^t (y_{\ell j} - y_{\ell j}^t)
	%		= \alpha_{\ell}^t y_{\ell j} + y_{\ell j}^t (\alpha_{\ell} - \alpha_{\ell}^t).
	%	\end{aligned}
%\end{equation}
%\todo[inline]{YW: How to introduce $t$ smoothly?\\
	%WZ:This is a recursion algorithm, so we can say given $y^t$}
%If $\sum_{j \in J} y_{\ell j}^t = 0$, then $\widehat{\alpha_{\ell} y_{\ell j}} = \alpha_{\ell}^t y_{\ell j}$ for all $j \in J$.
%\todo[inline]{YW: Add some description for this case: \\
	%When there is no flow at pool $\ell$, then $\widehat{\alpha_{\ell} y_{\ell j}}$ is equal to $\alpha_{\ell}^t y_{\ell j}$. 
	%But why should we justify the correctness/rationality of using $\alpha_{\ell}^t y_{\ell j}$ to further approximate $\widehat{\alpha_{\ell} y_{\ell j}}$, an approximation of bilinear $\alpha_{\ell} y_{\ell j}$?
	%Why don't we just use \eqref{1st-Taylor}? \\
	%Therefore, it is necessary to explain the disadvantage of using $y_{\ell j}^t$ compared to $\beta_{\ell j}^t$.
	%But we do not know the form of $\beta_{\ell j}^t$ at the beginning!\\
	%WZ: Here, we use \eqref{1st-Taylor} is to derive DR expre. So I think this part should be remove. Because next I have given why we have classification about \eqref{1st-Taylor}. And we can say the advantage at the red part.}
%In the following of this section, we assume that $\sum_{j \in J} y_{\ell j}^t > 0$.
%By substituting $\alpha_{\ell} y_{\ell j}$ by \eqref{1st-Taylor} for all $j \in J$, we can measure the error in the specification tracking constraint \eqref{cons:material-balance-ell} as 
%\begin{equation}\label{def:error-ell}
%	\begin{aligned}
	%		o_{\ell} 
	%		& = \sum_{j \in J} \widehat{\alpha_{\ell} y_{\ell j}} - \sum_{i \in I} \lambda_i y_{i \ell}\\
	%		& = \sum_{j \in J} \left(\alpha_{\ell}^t y_{\ell j} + y_{\ell j}^t (\alpha_{\ell} - \alpha_{\ell}^t)\right)
	%		- \sum_{i \in I} \lambda_{i} y_{i \ell} \\
	%		& = 
	%		\alpha_{\ell}^t \sum_{j \in J} y_{\ell j} 
	%		+ (\alpha_{\ell} - \alpha_{\ell}^t) \sum_{j \in J} y_{\ell j}^t 
	%		- \sum_{i \in I} \lambda_{i} y_{i \ell}.
	%	\end{aligned}
%\end{equation}
%From \eqref{def:error-ell} and $\sum_{j \in J} y_{\ell j}^t > 0$, we have 
%\begin{equation}\label{alpha-diff}
%	\alpha_{\ell} - \alpha_{\ell}^t =  \frac{ o_{\ell} +  \sum_{i \in I} \lambda_{i} y_{i \ell} - \alpha_{\ell}^t \sum_{j \in J} y_{\ell j} }{ \sum_{j \in J} y_{\ell j}^t}.
%\end{equation}
%Substituting $\alpha_{\ell} - \alpha_{\ell}^t$ by \eqref{alpha-diff} in \eqref{1st-Taylor} , we obtain
%\begin{equation*}
%	\widehat{\alpha_{\ell} y_{\ell j}} = \alpha_{\ell}^t y_{\ell j} + \frac{y_{\ell j}^t}{ \sum_{j \in J} y_{\ell j}^t} \left(o_{\ell} +  \sum_{i \in I} \lambda_{i} y_{i \ell} - \alpha_{\ell}^t \sum_{j \in J} y_{\ell j} \right).
%\end{equation*}
%By introducing variables 
%\begin{equation}\label{def:R}
%	R_{\ell k} = \red{o_{\ell}} + \sum_{i \in I} \lambda_{i} y_{i \ell} - \alpha_{\ell}^t \sum_{j \in J} y_{\ell j},
%\end{equation}
%\todo[inline]{YW: How to remove $o_{\ell}$? 
	%	That is how to justify why we should approximate $\widehat{\alpha_{\ell} y_{\ell j}}$?\\
	%	Advantage of using $\beta_{\ell j}^t$ and $R_{\ell k}$ instead of $\alpha_{\ell}$: when $\sum_{j \in J} y_{\ell j}^t$ is small, the value of $R_{\ell k}$ will also be small while $\alpha_{\ell}$ varies and could be any value (within the bound) (oscillation? sensitive?). 
	%	\begin{equation*}
		%		\alpha_{\ell} = \frac{\sum_{i \in I} \lambda_i y_{i \ell}  - \alpha_{\ell}^t \sum_{j \in J} (y_{\ell j} - y_{\ell j}^t)}{\sum_{\ell j}^t y_{\ell j}^t}
		%		\end{equation*}\\
	%	
	%WZ: unnecessary to introduce $o_{\ell}$, you should say according to Tylor series, for the constraint \eqref{cons:material-balance-ell-layer}, we  also have:
	%\begin{equation}
	%	\sum_{i \in I} \lambda_{ik}y_{i\ell} = \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j} + \sum_{j \in J} y_{\ell j}^{t} \Delta \alpha_{\ell k}.
	%\end{equation}   }
	%and distribution coefficients
	%\begin{equation}\label{def:beta}
	%	\beta_{\ell j}^t = \left\{
	%	\begin{aligned}
		%		& \frac{y_{\ell j}^t}{\sum_{j \in J} y_{\ell j}^t} && \text{ if } \sum_{j \in J} y_{\ell j}^t > 0;\\
		%		& 0 && \text{ otherwise},
		%	\end{aligned}
	%	\right.
	%\end{equation}
	%the first Taylor polynomials can be uniformly represented as
	%\begin{equation*}
	%	\widehat{\alpha_{\ell} y_{\ell j}} = \alpha_{\ell}^t y_{\ell j} + \beta_{\ell j}^t R_{\ell k}.
	%\end{equation*}
	%\todo[inline]{YW: 1. The rest of this section has not been revised.\\
		%2. The subscripts in the above text need to be checked.}
	
	
	
	
	
	
	
	%Next, we introduce how to derive the DR method 
	%in mathematics. At the iteration point $y^t$, if there has mixing occurs at node $\ell \in L$, we can calculate the $\alpha^t$ according to \eqref{cons:material-balance-ell}. That is:
	%\begin{equation}
	%	\alpha_{\ell k}^t = 
	%	\begin{aligned}
		%		& \frac{\sum_{i \in I} \lambda_{ik} y_{i\ell}^t}{\sum_{j \in J}y_{\ell j}^t},  
		%	\end{aligned}\forall \ \ell \in L, \ k \in K.
	%\end{equation}
	%In the absence of any mixing, we shall refrain from taking any action. However, we initially postulate that mixing occurs at the every node.
	
	%\todo[inline]{WF: Here are some commits, see ".tex" for details}
	% （10）和（11）不需要，之前提过。并且直接考虑这两个太突然。
	% 先说明pooling问题中 alpha*y 是仅有的非线性项，我们考虑他们的一阶近似。
	% 然后得到了（12）
	% 把（12）的近似结果带入原问题，得到了（13）和（14）
	% 汇总之后得到了问题（1）的LP模型（15）
	
	% 接下来说DR模型中的LP子问题，与（15）不一样。再具体说DR是怎么来的
	% 在命题4.1前，先说明这两个子模型的异同，包括：
	% 参数的更新、解的异同。由此引出命题4.1。
	
	% （24,25,26）更新前，先说明根据DR子问题得到了估计点y_{k+1}
	% （24,25,26）的更新上标写成 k+1
	% ========================================
	%As is mentioned in Section  \eqref{section:3}, the bilinear term  $\alpha_{\ell k}y_{\ell j},\forall \ j \in J, k\in K, $ in \eqref{prob:pooling-P} makes it a nonconvex and nonlinear optimization problem. To approximating the  the nonlinear term as a linear term, given iteration point $(y^t, \alpha^t)$, we have the first-order Taylor expansion of the term:
	%\begin{equation}
	%	\begin{aligned} \label{term-linear}
		%		\alpha_{\ell k}y_{\ell j}\approx 
		%		&\alpha_{\ell k}^t y_{\ell j}^t + \left.\frac{\partial (\alpha_{\ell k} y_{\ell j})}{\partial y_{\ell j}}\right|_{(y^t, \alpha^t)} (y_{\ell j} - y^t_{\ell j} ) + \frac{\partial (\alpha_{\ell k} y_{\ell j})}{\partial \alpha_{\ell k}}|_{(y^t, \alpha^t)} (\alpha_{\ell k} - \alpha^t_{\ell k} )\\
		%		= &\alpha_{\ell k}^t y_{\ell j}^t +  \alpha_{\ell k}^t (y_{\ell j} - y^t_{\ell j} ) + y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k} )\\
		%		= &\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k}).
		%	\end{aligned}
	%\end{equation}
	%Then nonlinear constraint \eqref{cons:material-balance-ell} has the linear approximatin at $(y^t,\alpha^t)$:
	%\begin{equation}\label{cons:material-balance-ell-layer-LP}
	%	\sum_{i \in I} \lambda_{ik} y_{i\ell} 
	%	=  \sum_{j \in J} (\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k})), \ \forall \ \ell \in L, k \in K,
	%\end{equation}
	%and \eqref{cons:material-balance-j-all} becomes:
	%\begin{subequations}\label{cons:material-balance-j-all-LP}\begin{align}
	%		& \sum_{i \in I} \lambda_{ik} y_{ij}
	%		+ \sum_{\ell \in L} (\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k})) \ge \lambda_{jk}^{\min} \sum_{i \in I \cup L} y_{ij},\ \forall \ j \in J, \ k \in K,\\
	%		& \sum_{i \in I} \lambda_{ik} y_{ij}
	%		+ \sum_{\ell \in L} (\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k})) \le 	\lambda_{jk}^{\max} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K.
	%\end{align}\end{subequations}
	%
	%So for problem \eqref{prob:pooling-P}, we have a LP subproblem:
	%\begin{equation}\label{prob:pooling-P-LP}
	%	\begin{aligned}
		%		\max_{y,\alpha}\ & \sum_{j \in J} c_j \sum_{i \in I \cup L}  y_{ij} - \sum_{i \in I} c_i \sum_{j \in L \cup J}y_{ij} \\
		%		\text{s.t.}
		%		&\eqref{cons:material-balance-ell-layer-LP},\eqref{cons:material-balance-j-all-LP},\\
		%		&\eqref{cons:flow-conservation},
		%		\eqref{cons:capacity-node-i},
		%		\eqref{cons:capacity-node-ell},
		%		\eqref{cons:capacity-node-j},
		%		\eqref{cons:capacity-arc}.
		%	\end{aligned}
	%\end{equation}
	%For the constraint \eqref{cons:material-balance-ell-layer-LP} in this LP subproblem,
	%$\text{if} \ \sum_{j\in J} y_{\ell j}^t > 0,$ then we can rewrite it as:
	%\begin{equation}\label{tmpeq1}
	%	\alpha_{\ell k} - \alpha^t_{\ell k} = \frac{\sum_{i \in I} \lambda_{ik}y_{i\ell}- \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j}}{ \sum_{j \in J} y_{\ell j}^t}.
	%\end{equation}
	%Bring it in \eqref{term-linear}, we obtain:
	%\begin{equation}\label{tmpeq2}
	%	\begin{aligned} 
		%		&\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k})\\
		%		=&\alpha_{\ell k}^t y_{\ell j} + \frac{y_{\ell j}^t (\sum_{i \in I} \lambda_{ik}y_{i\ell} - \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j})}{ \sum_{j \in J} y_{\ell j}^t}\\
		%		=&\alpha_{\ell k}^t y_{\ell j} +  \beta_{\ell j}^t R_{\ell k}.\\
		%	\end{aligned}
	%\end{equation}
	%Here, $\beta_{\ell j}^t :=\frac{y_{\ell j}^t }{ \sum_{j \in J} y_{\ell j}^t}$, $ R_{\ell k} := \sum_{i \in I} \lambda_{ik}y_{i\ell} - \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j}.$ Otherwise, if  $\sum_{j\in J}y_{\ell j}^t = 0$, we set $\beta_{\ell j}^t =0, \forall \ j \in J$.
	%%\todo[inline]{YW@WZ: Parameters $\beta$ and variables $R$ to ``unify'' the different forms of $\alpha_{\ell k}^t y_{\ell j} +  y_{\ell j}^t  (\alpha_{\ell k} - \alpha^t_{\ell k})$ after removing $\alpha_{\ell k}$. 
		%%(I have written a version but it is not presented here.)\\
		%%Please revise this part (how to present $\beta$ and $R$) according to the what I wrote.
		%%And do not change what I wrote without asking me because, otherwise, I have to write it again and again.\\
		%%\blue{By introducing variables 
			%%\begin{equation}\label{def:R}
			%%	R_{\ell k} =  \sum_{i \in I} \lambda_{i} y_{i \ell} - \alpha_{\ell}^t \sum_{j \in J} y_{\ell j},
			%%\end{equation}
			%%and distribution coefficients
			%%\begin{equation}\label{def:beta}
			%%	\beta_{\ell j}^t = \left\{
			%%	\begin{aligned}
				%%			& \frac{y_{\ell j}^t}{\sum_{j \in J} y_{\ell j}^t} && \text{ if } \sum_{j \in J} y_{\ell j}^t > 0;\\
				%%			& 0 && \text{ otherwise},
				%%		\end{aligned}
			%%	\right.
			%%\end{equation}
			%%the first Taylor expansion $\alpha_{\ell k}^t + y_{\ell j}^t (\alpha_{\ell k} - \alpha_{\ell k}^t)$ can be uniformly represented as
			%%\begin{equation}\label{each-bilinear-betaR}
			%%	\alpha_{\ell k}^t + y_{\ell j}^t (\alpha_{\ell k} - \alpha_{\ell k}^t) = \alpha_{\ell}^t y_{\ell j} + \beta_{\ell j}^t R_{\ell k}.
			%%\end{equation}}
			%%} 
		%
		%Then constrains \eqref{cons:material-balance-ell-layer-LP}  and \eqref{cons:material-balance-j-all-LP} are reformulated as:
		%\begin{align}\label{cons:material-balance-ell-layer-linear}
		%%		\left\{
		%%	\begin{array}{ll}
			%%		\sum_{i \in I} \lambda_{ik} y_{i\ell} 
			%%		= \alpha_{\ell k}^t \sum_{j \in J} y_{\ell j} + R_{\ell k},& \text{if} \ \sum_{j \in  J} y_{\ell j}^t > 0,\\
			%%		\sum_{i \in I} \lambda_{ik} y_{i\ell} 
			%%	= \alpha_{\ell k}^t \sum_{j \in J} y_{\ell j},  &\text{otherwise},
			%%	\end{array}
		%%	\right.
		%\sum_{i \in I} \lambda_{ik} y_{i\ell} 
		%		= \alpha_{\ell k}^t \sum_{j \in J} y_{\ell j} + R_{\ell k}\sum_{j\in J} \beta_{\ell j}^t,
		%	\ \forall \ \ell \in L, k \in K,
		%\end{align}
		%and
		%\begin{subequations}\label{cons:material-balance-j-all-linear}
		%	\begin{align}
			%		& \sum_{i \in I} \lambda_{ik} y_{ij}
			%		+ \sum_{\ell \in L}( \alpha_{\ell k}^t y_{\ell j} +  \beta_{\ell j}^t R_{\ell k}) \ge 	\lambda_{jk}^{\min} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K,\\
			%		&\sum_{i \in I} \lambda_{ik} y_{ij}
			%		+ \sum_{\ell \in L} (\alpha_{\ell k}^t y_{\ell j} +  \beta_{\ell j}^t R_{\ell k}) \le 	\lambda_{jk}^{\max} \sum_{i \in I \cup L} y_{ij}, \ \forall \ j \in J, \ k \in K,
			%	\end{align}
		%\end{subequations}
		%respectively. Therefore, we have the LP subproblem for the  DR approach: 
		%\begin{equation}\label{prob:pooling-P-DR}
		%	\begin{aligned}
			%		\max_{y,R}\ & \sum_{j \in J} c_j \sum_{i \in I \cup L}  y_{ij} - \sum_{i \in I} c_i \sum_{j \in L \cup J}y_{ij}  \\
			%		\text{s.t.}
			%		&\eqref{cons:material-balance-ell-layer-linear}, \eqref{cons:material-balance-j-all-linear}\\
			%		&
			%	\eqref{cons:flow-conservation},
			%	\eqref{cons:capacity-node-i},
			%	\eqref{cons:capacity-node-ell},
			%	\eqref{cons:capacity-node-j},
			%	\eqref{cons:capacity-arc}.
			%	\end{aligned}
		%\end{equation}
		%\begin{proposition} \label{proposition}
		%The feasible region of Model \eqref{prob:pooling-P-DR} is a strict superset of the feasible region of Model \eqref{prob:pooling-P-LP}.
		%\end{proposition}
		%\begin{proof}
		%Consider any feasible point $(y, \alpha)$ in the model \eqref{prob:pooling-P-LP}. We want to show that there exists a $R$ such that the point $(y, R)$ satisfies the constraints \eqref{cons:material-balance-ell-layer-linear} and \eqref{cons:material-balance-j-all-linear}.
		%
		%Observe that the expression for $R_{\ell k}$ is given by:
		%\begin{equation}
		%	R_{\ell k} = \sum_{i \in I} \lambda_{ik}y_{i\ell} - \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j}, \quad \forall \ell \in L, k \in K
		%\end{equation}
		%Substituting this expression into the constraint \eqref{cons:material-balance-ell-layer-linear}, we can see that it is trivially satisfied, as it reduces to the identity $0 = 0$. Therefore, the constraint \eqref{cons:material-balance-ell-layer-linear} is naturally satisfied for any feasible point $(y, \alpha)$.
		%
		%Now, consider the constraint \eqref{cons:material-balance-j-all-linear}. For any $j \in J$, if $y_{\ell j}^t = 0$, then \eqref{cons:material-balance-j-all-LP} and \eqref{cons:material-balance-j-all-linear} are identical. If $y_{\ell j}^t > 0$, then \eqref{cons:material-balance-ell-layer-LP} implies:
		%\begin{equation}
		%	\alpha_{\ell k} - \alpha^t_{\ell k} = \frac{\sum_{i \in I} \lambda_{ik}y_{i\ell} - \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j}}{\sum_{j \in J} y_{\ell j}^t}
		%\end{equation}
		%Substituting this expression into \eqref{term-linear}, we can derive the constraint \eqref{cons:material-balance-j-all-linear}. Therefore, the constraint \eqref{cons:material-balance-j-all-linear} is also satisfied for any feasible point $(y, \alpha)$.
		%
		%Next, we consider the reverse direction. If we have a feasible point $(y, R)$ in the model \eqref{prob:pooling-P-DR}. We want to show that there exists an $\alpha$ such that the point $(y, \alpha)$ satisfies the constraints \eqref{cons:material-balance-ell-layer-LP} and \eqref{cons:material-balance-j-all-LP}. Suppose there exists a feasible solution $(y,R)$ of model \eqref{prob:pooling-P-DR} and $R > 0$, so \eqref{cons:material-balance-ell-layer-linear} satisfies:
		%\begin{equation}
		%	 \sum_{i \in I} \lambda_{ik}y_{i\ell} = \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j} + R_{\ell k}, \quad \forall \ell \in L, k \in K
		%\end{equation}
		%Now, let us consider a special case, where exists a parameter $(y^t, \alpha^t)$ such that $y^t = 0$ and $\alpha^t > 0$. Then \eqref{cons:material-balance-ell-layer-LP} becomes:
		%
		%\begin{equation}\label{cons:material-balance-ell-layer-LP-y0}
		%	\sum_{i \in I} \lambda_{ik} y_{i\ell} 
		%	=  \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j}, \ \forall \ \ell \in L, k \in K.
		%\end{equation}
		%However, no matter what the value of $\alpha$,  \eqref{cons:material-balance-ell-layer-LP-y0} is not is not satisfied, this is a 
		%contradiction. 
		%
		%
		%
		%%Suppose there exists a feasible point $(y, R)$ in \eqref{prob:pooling-P-DR}. Then, for all $\ell \in L$ and $k \in K$, the expression for $R_{\ell k}$ is given by $\alpha_{\ell k}$ according to the Taylor expansion:
		%%\begin{subequations}
		%%	\begin{align}
			%%		R_{\ell k} &= \sum_{i \in I} \lambda_{ik}y_{i\ell} - \alpha_{\ell k}^t\sum_{j \in J} y_{\ell j} \\
			%%		&= \sum_{j \in J} y_{\ell j}^{t} (\alpha_{\ell k} - \alpha^t_{\ell k}) + \sum_{j \in J}(\alpha_{\ell k} - \alpha^t_{\ell k})(y_{\ell j}-y_{\ell j}^{t})
			%%	\end{align}
		%%\end{subequations}
		%%and the point $(y, \alpha)$ satisfies $\sum_{j \in J}(\alpha_{\ell k} - \alpha^t_{\ell k})(y_{\ell j}-y_{\ell j}^{t}) > 0$. However, this point $(y, \alpha)$ does not satisfy the constraints \eqref{cons:material-balance-ell-layer-LP}. Therefore, the point $(y, R)$ is not a feasible solution in  the  model \eqref{prob:pooling-P-LP}, it is a contradiction.
		%
		%The proof is now complete. 
		%\end{proof}
		
		%The solutions $y$ of LP subproblem \eqref{prob:pooling-P-LP} and \eqref{prob:pooling-P-DR} are the same according to the reformulations we concerned above. However,
		%the updating rules of $\alpha$ would result in the main difference between SLP and DR approach.
		%In SLP apporach, the next iterative point $\alpha^{t+1}$  satisfies the constraint \eqref{cons:material-balance-ell-layer-LP} of \eqref{prob:pooling-P-LP}; in DR approach, after we get a solution $y^{t+1}$ of \eqref{prob:pooling-P-DR}, we update $\alpha^{t+1}$ such that it satisfies the real physical meaning:
		%\begin{equation}
		%	\sum_{i \in I} \lambda_{ik}y_{i\ell}^{t+1} = \alpha_{\ell k}^{t+1}\sum_{j \in J} y_{\ell j}^{t+1} .
		%\end{equation} 
		%
		%In conclusion, the parameters $\alpha^{t+1}$ and $\beta^{t+1}$ in DR approach are updated as follows:
		%\begin{align}\label{alpha_renew}
		%	&\alpha_{\ell k}^{t+1} = 
		%	\left\{
		%	\begin{array}{ll}
			%		\frac{\sum_{i \in I} \lambda_{ik}y_{i\ell}^{t+1} }{\sum_{j \in  J} y_{\ell j}^{t+1}},& \text{if} \ \sum_{j \in  J} y_{\ell j}^{t+1} > 0,\\
			%		\alpha^{t},  &\text{if} \ \sum_{j \in  J} y_{\ell j}^{t+1} = 0,
			%	\end{array}
		%	\right.
		%	 \forall \ \ell \in L, \ k \in K;\\ \label{beta_renew}
		%	&\beta_{\ell j}^{t+1} = 
		%	\left\{
		%	\begin{array}{ll}
			%		\frac{y_{i\ell}^{t+1} }{\sum_{j \in  J} y_{\ell j}^{t+1}},& \text{if} \ \sum_{j \in  J} y_{\ell j}^{t+1} > 0,\\
			%		0,  &\text{otherwise,} \ 
			%	\end{array}
		%	\right.
		%	 \forall \ \ell \in L, \ j \in J.
		%\end{align}


==> table/T2-1.tex <==
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrc@{}}
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{\tblid}}
	&\multicolumn{5}{c}{\testSLP}
	&\multicolumn{5}{c}{\testDR}
	&\multicolumn{5}{c}{\testPDR}
	&\multicolumn{3}{c}{\testGRB}
	\\
	\cmidrule(r){2-6}\cmidrule(r){7-11}\cmidrule(r){12-16}\cmidrule(r){17-19}
	
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblGap}
	\\\midrule
	A1-3-2-3-2          	& $<0.01$	&  160.71	&       2	&    73.8	&    13.5	& $<0.01$	&  612.94	&       3	&     0.0	&    71.6	& $<0.01$	&  612.94	&       4	&     0.0	&    91.4	&    0.08	&  612.94	&     0.0\\ 
	A2-3-2-3-2          	& $<0.01$	&  250.00	&       2	&    43.8	&    34.2	& $<0.01$	&  250.00	&      10	&    43.8	&    47.6	& $<0.01$	&  415.00	&       7	&     6.7	&    47.6	&   61.42	&  445.00	&     0.0\\ 
	A3-3-2-3-2          	& $<0.01$	&  236.62	&       2	&     3.7	&    58.7	& $<0.01$	&  245.73	&       4	&     0.0	&    72.6	&    0.04	&  245.73	&     100	&     0.0	&    72.6	&    0.29	&  245.73	&     0.0\\ 
	A4-3-2-3-2          	& $<0.01$	&  403.10	&       2	&    36.3	&    54.5	& $<0.01$	&  632.70	&       7	&     0.0	&    91.2	& $<0.01$	&  632.70	&       5	&     0.0	&    92.9	&    0.38	&  632.70	&     0.0\\ 
	A5-3-2-3-2          	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&    0.00	&       3	&   100.0	&    50.0	& $<0.01$	&  280.29	&       4	&     0.0	&    96.2	&    0.15	&  280.29	&     0.0\\ 
	A6-3-2-3-2          	& $<0.01$	&  530.84	&       3	&     0.0	&    51.8	&    0.01	&  530.84	&      11	&     0.0	&    60.4	& $<0.01$	&  510.32	&       4	&     3.9	&    71.0	&    0.11	&  530.84	&     0.0\\ 
	A7-3-2-3-2          	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&  341.00	&       4	&     0.0	&    72.0	&    0.20	&  341.00	&     0.0\\ 
	A8-3-2-3-2          	& $<0.01$	& 1536.00	&       2	&     9.9	&    86.3	& $<0.01$	& 1704.00	&       4	&     0.0	&    97.0	& $<0.01$	& 1704.00	&       4	&     0.0	&    97.0	&    2.44	& 1704.00	&     0.0\\ 
	A9-3-2-3-2          	& $<0.01$	&  994.50	&       4	&     5.5	&    87.1	& $<0.01$	& 1052.50	&       4	&     0.0	&    92.4	& $<0.01$	& 1052.50	&       4	&     0.0	&    92.4	&    0.29	& 1052.50	&     0.0\\ 
	A10-3-2-3-2         	& $<0.01$	&  135.00	&       2	&    77.9	&     7.4	& $<0.01$	&  612.00	&       3	&     0.0	&    55.3	& $<0.01$	&  612.00	&       3	&     0.0	&    55.3	&    0.12	&  612.00	&     0.0\\ 
	B1-5-4-3-3          	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&   97.50	&       5	&    70.9	&    94.8	& $<0.01$	&   97.50	&       5	&    70.9	&    94.8	&\texttt{TL}	&  335.00	&     0.0\\ 
	B2-5-4-3-3          	& $<0.01$	&  300.00	&       2	&    66.9	&    27.6	& $<0.01$	&  905.25	&       5	&     0.0	&    88.1	& $<0.01$	&  905.25	&       5	&     0.0	&    88.1	&\texttt{TL}	&  905.25	&     0.0\\ 
	B3-5-4-3-3          	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&  159.71	&       4	&     0.0	&    65.6	& $<0.01$	&  159.71	&       8	&     0.0	&    65.6	&\texttt{TL}	&  159.71	&     0.0\\ 
	B4-5-4-3-3          	& $<0.01$	&  668.67	&      18	&     5.5	&    80.5	& $<0.01$	&  674.41	&      12	&     4.7	&    85.6	& $<0.01$	&  675.33	&       6	&     4.5	&    85.5	&    0.72	&  707.33	&     0.0\\ 
	B5-5-4-3-3          	& $<0.01$	&  459.43	&       2	&    16.3	&    33.7	& $<0.01$	&  470.40	&       4	&    14.3	&    76.1	& $<0.01$	&  470.40	&       4	&    14.3	&    76.1	&\texttt{TL}	&  548.57	&     0.0\\ 
	B6-5-4-3-3          	& $<0.01$	&  795.00	&       2	&    23.7	&    63.4	& $<0.01$	&  823.20	&       6	&    21.0	&    85.9	& $<0.01$	&  823.20	&       8	&    21.0	&    90.2	&\texttt{TL}	& 1042.55	&     0.0\\ 
	B7-5-4-3-3          	& $<0.01$	&  638.00	&       3	&    57.7	&    52.9	& $<0.01$	& 1028.00	&       4	&    31.9	&    89.4	& $<0.01$	& 1028.00	&       5	&    31.9	&    93.5	&  336.62	& 1509.00	&     0.0\\ 
	B8-5-4-3-3          	& $<0.01$	&  663.00	&       2	&    33.7	&    49.1	& $<0.01$	& 1000.00	&       8	&     0.0	&    93.9	& $<0.01$	& 1000.00	&      12	&     0.0	&    93.9	&\texttt{TL}	& 1000.00	&     0.0\\ 
	B9-5-4-3-3          	& $<0.01$	&  352.00	&       2	&    29.6	&    24.6	& $<0.01$	&  499.69	&       7	&     0.0	&    95.7	& $<0.01$	&  499.69	&       7	&     0.0	&    95.7	&\texttt{TL}	&  499.69	&     0.0\\ 
	B10-5-4-3-3         	& $<0.01$	&  827.40	&       8	&     4.7	&    67.8	& $<0.01$	&  868.00	&      14	&     0.0	&    85.9	& $<0.01$	&  868.00	&      10	&     0.0	&    82.6	&    0.01	&  868.00	&     0.0\\ 
	C1-8-6-6-4          	&    0.09	&     ---	&     100	&     ---	&    77.8	&    0.15	& 1828.07	&      83	&     0.0	&    85.2	&    0.02	& 1828.07	&      12	&     0.0	&    85.2	&\texttt{TL}	& 1828.07	&     0.0\\ 
	C2-8-6-6-4          	&    0.17	&     ---	&     100	&     ---	&    47.5	&    0.10	& 1011.54	&      46	&    19.1	&    62.2	&    0.02	& 1011.54	&      14	&    19.1	&    65.4	&\texttt{TL}	& 1250.97	&     0.0\\ 
	C3-8-6-6-4          	&    0.10	&     ---	&     100	&     ---	&    73.2	&    0.02	& 1273.58	&      15	&    23.1	&    65.8	&    0.05	& 1273.58	&      39	&    23.1	&    76.7	&\texttt{TL}	& 1656.52	&     0.0\\ 
	C4-8-6-6-4          	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	& $<0.01$	&  220.80	&       6	&     6.2	&   100.0	& $<0.01$	&  220.80	&       5	&     6.2	&   100.0	&\texttt{TL}	&  235.42	&     0.0\\ 
	C5-8-6-6-4          	&    0.12	&     ---	&     100	&     ---	&    22.9	&    0.02	&  653.55	&      16	&     0.0	&    43.0	&    0.04	&  653.55	&      33	&     0.0	&    44.9	&\texttt{TL}	&  652.48	&     0.2\\ 
	\bottomrule
\end{tabular}


==> table/T2-2.tex <==
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrc@{}}
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{\tblid}}
	&\multicolumn{5}{c}{\testSLP}
	&\multicolumn{5}{c}{\testDR}
	&\multicolumn{5}{c}{\testPDR}
	&\multicolumn{3}{c}{\testGRB}
	\\
	\cmidrule(r){2-6}\cmidrule(r){7-11}\cmidrule(r){12-16}\cmidrule(r){17-19}
	
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblIter}&\multicolumn{1}{c}{\tblGap}&\multicolumn{1}{c}{\tblObjAver}
	&\multicolumn{1}{c}{\tblT}&\multicolumn{1}{c}{\tblObj}&\multicolumn{1}{c}{\tblGap}
	\\\midrule
	C6-8-6-6-4          	& $<0.01$	& 1056.49	&       2	&     2.7	&    40.8	& $<0.01$	& 1085.33	&       6	&     0.0	&    91.3	& $<0.01$	& 1085.33	&       6	&     0.0	&    91.3	&\texttt{TL}	& 1082.92	&     0.2\\ 
	C7-8-6-6-4          	&    0.03	&  584.29	&      26	&    48.7	&    30.1	&    0.03	& 1139.93	&      28	&     0.0	&    62.8	&    0.01	& 1139.93	&      10	&     0.0	&    60.9	&\texttt{TL}	& 1132.68	&     0.6\\ 
	C8-8-6-6-4          	&    0.02	& 1303.20	&      19	&    21.3	&    63.3	&    0.03	& 1303.20	&      31	&    21.3	&    69.7	&    0.02	& 1303.20	&      17	&    21.3	&    71.7	&\texttt{TL}	& 1655.83	&     0.0\\ 
	C9-8-6-6-4          	&    0.05	&  780.13	&      36	&    39.8	&    64.7	& $<0.01$	& 1295.22	&       5	&     0.0	&    80.7	& $<0.01$	& 1192.98	&       4	&     7.9	&    79.4	&\texttt{TL}	& 1292.55	&     0.2\\ 
	C10-8-6-6-4         	& $<0.01$	& 2635.85	&       5	&     2.3	&    78.1	&    0.04	& 2698.76	&      35	&     0.0	&    85.8	&    0.02	& 2698.76	&      13	&     0.0	&    85.6	&\texttt{TL}	& 2698.76	&     0.0\\ 
	D1-12-10-8-5        	&    0.18	&     ---	&     100	&     ---	&    99.8	&    0.01	& 3006.86	&       6	&     0.2	&    99.9	&    0.01	& 3006.86	&       6	&     0.2	&    99.9	&   13.77	& 3013.00	&     0.0\\ 
	D2-12-10-8-5        	&    0.04	&  540.00	&      14	&    60.4	&    30.5	&    0.01	&  540.00	&       7	&    60.4	&    54.7	&    0.04	&  540.00	&       9	&    60.4	&    69.2	&\texttt{TL}	& 1364.01	&     0.0\\ 
	D3-12-10-8-5        	&    0.25	&     ---	&     100	&     ---	&    83.0	&    0.16	& 2343.06	&      50	&     7.1	&    83.4	&    0.35	& 2521.03	&     100	&     0.0	&    84.9	&\texttt{TL}	& 2521.03	&     0.0\\ 
	D4-12-10-8-5        	&    0.31	&     ---	&     100	&     ---	&    10.3	& $<0.01$	&  270.05	&       5	&    73.4	&    44.9	&    0.02	&  270.05	&      11	&    73.4	&    45.5	&\texttt{TL}	& 1013.98	&     0.0\\ 
	D5-12-10-8-5        	&    0.26	&     ---	&     100	&     ---	&    77.1	&    0.47	&     ---	&     100	&     ---	&    87.6	&    0.51	&     ---	&     100	&     ---	&    87.6	&\texttt{TL}	& 2949.09	&     0.0\\ 
	D6-12-10-8-5        	&    0.13	& 1114.17	&      33	&    41.4	&    41.4	&    0.49	&     ---	&     100	&     ---	&    72.4	&    0.63	&     ---	&     100	&     ---	&    72.5	&\texttt{TL}	& 1901.61	&     0.0\\ 
	D7-12-10-8-5        	&    0.27	&     ---	&     100	&     ---	&    59.0	&    0.40	&     ---	&     100	&     ---	&    63.1	&    0.48	&     ---	&     100	&     ---	&    62.5	&\texttt{TL}	& 2204.61	&     0.0\\ 
	\red{D8-12-10-8-5}        	&    0.16	&     ---	&     100	&     ---	&    69.5	&    0.24	&     ---	&     100	&     ---	&    91.6	&    0.03	& 3500.48	&      10	&     0.0	&    94.2	&\texttt{TL}	& 3357.58	&     \red{4.1}\\ 
	D9-12-10-8-5        	&    0.18	&     ---	&     100	&     ---	&    20.1	&    0.03	&  785.53	&      16	&     0.0	&    34.8	&    0.08	&  785.53	&      44	&     0.0	&    34.9	&\texttt{TL}	&  782.89	&     0.3\\ 
	D10-12-10-8-5       	&    0.22	&     ---	&     100	&     ---	&    71.8	&    0.07	& 3025.13	&      41	&     0.0	&    79.8	&    0.13	& 3025.13	&      49	&     0.0	&    86.9	&\texttt{TL}	& 3025.13	&     0.0\\ 
	E1-10-10-15-12      	&    0.10	&  317.47	&      17	&     3.3	&     4.4	&    0.02	&  328.17	&       5	&     0.0	&    43.1	&    0.04	&  328.17	&       8	&     0.0	&    44.9	&\texttt{TL}	&  328.17	&     0.0\\ 
	\red{E2-10-10-15-12}      	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	&    0.03	&  728.99	&       5	&     0.0	&   100.0	&    0.05	&  728.99	&       7	&     0.0	&   100.0	&\texttt{TL}	&  331.50	&    \red{54.5}\\ 
	E3-10-10-15-12      	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	&    0.03	&    0.00	&       5	&   100.0	&    88.8	&    0.08	&  171.37	&       6	&     0.0	&    88.8	&\texttt{TL}	&  171.37	&     0.0\\ 
	E4-10-10-15-12      	& $<0.01$	&  260.67	&       2	&     1.4	&     4.4	&    0.05	&  264.50	&       9	&     0.0	&    83.7	&    0.08	&  264.50	&       7	&     0.0	&    83.7	&\texttt{TL}	&  264.50	&     0.0\\ 
	\red{E5-10-10-15-12}      	&    0.75	&     ---	&     100	&     ---	&     6.0	&    0.03	&  396.41	&       5	&     0.0	&    38.1	&    0.07	&  396.41	&      11	&     0.0	&    41.9	&\texttt{TL}	&  383.20	&     \red{3.3}\\ 
	E6-10-10-15-12      	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	&    0.04	&    0.00	&       5	&   100.0	&   100.0	&    0.06	&  498.72	&       7	&     0.0	&   100.0	&\texttt{TL}	&  498.72	&     0.0\\ 
	E7-10-10-15-12      	& $<0.01$	&    0.00	&       2	&   100.0	&     0.0	&    0.03	&    0.00	&       6	&   100.0	&   100.0	&    0.06	&  635.51	&       9	&     0.0	&   100.0	&\texttt{TL}	&  635.51	&     0.0\\ 
	E8-10-10-15-12      	&    0.05	&  386.22	&       7	&    56.0	&     9.9	&    0.04	&  386.22	&       5	&    56.0	&    61.2	&    0.14	&  876.89	&      19	&     0.0	&    67.3	&\texttt{TL}	&  876.89	&     0.0\\ 
	\red{E9-10-10-15-12}      	&    0.01	&    0.00	&       2	&   100.0	&     0.0	&    0.03	&  323.88	&       4	&     0.0	&    89.7	&    0.07	&  323.88	&      12	&     0.0	&    89.7	&\texttt{TL}	&    0.00	&   \red{100.0}\\ 
	E10-10-10-15-12     	& $<0.01$	&  299.22	&       2	&     3.6	&     5.0	&    0.02	&  310.37	&       5	&     0.0	&    92.9	&    0.04	&  310.37	&       7	&     0.0	&    92.9	&\texttt{TL}	&  310.37	&     0.0\\ 
	\hline
	\multicolumn{1}{l}{\tblAve}
	&    0.07	&        	&    30.8	&    35.4	&    37.7	&    0.05	&        	&    19.4	&    19.1	&    75.1	&    \red{0.07}	&        	&    19.7	&     7.3	&    79.3	&        	&        	&     3.3\\ 
	\bottomrule
\end{tabular}


